Where is the answer? Investigating Positional Bias in Language Model Knowledge Extraction

Large language models require updates to remain up-to-date or adapt to new domains by fine-tuning them with new documents. One key is memorizing the latest information in a way that the memorized information is extractable with a query prompt. However, LLMs suffer from a phenomenon called perplexity curse; despite minimizing document perplexity during fine-tuning, LLMs struggle to extract information through a prompt sentence. In this new knowledge acquisition and extraction, we find a very intriguing fact that LLMs can accurately answer questions about the first sentence, but they struggle to extract information described in the middle or end of the documents used for fine-tuning. Our study suggests that the auto-regressive training causes this issue; each token is prompted by reliance on all previous tokens, which hinders the model from recalling information from training documents by question prompts. To conduct the in-depth study, we publish both synthetic and real datasets, enabling the evaluation of the QA performance w.r.t. the position of the corresponding answer in a document. Our investigation shows that even a large model suffers from the perplexity curse, but regularization such as denoising auto-regressive loss can enhance the information extraction from diverse positions. These findings will be (i) a key to improving knowledge extraction from LLMs and (ii) new elements to discuss the trade-off between RAG and fine-tuning in adapting LLMs to a new domain.

==> figures/ex_answers.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.7\textwidth]{images/example_synth_answer.pdf}
\vspace{-4mm}
    \caption{QA example in synthetic dataset.}
    \label{fig:answer_ex_synth}
\end{figure}

\begin{figure}[t]
    \centering
\includegraphics[width=0.7\textwidth]{images/example_answer_paper.pdf}
\vspace{-4mm}
    \caption{QA example in Paper2023 dataset.}
    \label{fig:answer_ex_paper}
\end{figure}

\begin{figure}[t]
    \centering
\includegraphics[width=0.7\textwidth]{images/examle_answer_news.pdf}
\vspace{-4mm}
    \caption{QA example in News2023 dataset.}
    \label{fig:answer_ex_news}
\end{figure}

==> figures/ex_papers.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.48\textwidth]{images/papers_example.pdf}
\vspace{-8mm}
    \caption{Example of a prompt, target sentences  (sentences to predict given prompt), and questions from Paper2023 dataset. For simplicity, we illustrate only three items, \ie, dataset, empirical results, and availability of the code.}
    \label{fig:paper_example}
\end{figure}

==> figures/ex_prompt_dataset.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.48\textwidth]{images/prompt_answer_dataset.pdf}
    \caption{Example of a prompt given to ChatGPT to obtain answer about the dataset used for evaluation.}
    \label{fig:prompt_ex_dataset}
\end{figure}

==> figures/ex_prompt_number.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.48\textwidth]{images/prompt_answer_number.pdf}
    \caption{Example of a prompt given to ChatGPT to generate a question and an answer pair about the given passage.}
    \label{fig:prompt_ex_number}
\end{figure}

==> figures/figure1.tex <==
\begin{figure}
    \centering
\includegraphics[width=0.5\textwidth]{images/fig1_v6.pdf}
\vspace{-5mm}
    \caption{Unlike the standard fine-tuning for LLM (top), our task (bottom) aims to adapt LLM model to a new domain in an unsupervised manner, \ie, training a model without using QA pairs from the domain. Instead, we employ a general QA dataset as the source data, which avoids incurring any annotation costs, resulting in the annotation-efficient setting.}
    \label{fig:teaser}
\end{figure}

==> figures/title_paper.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.45\textwidth]{images/qa_wo_title.png}
\vspace{-5mm}
    \caption{\textbf{The effectiveness of prompting with the paper title for Paper2023.} Y-axis shows the percentage of answers judged as correct or partially correct. If queries do not include the paper title, the performance of answering the queries significantly degrades. }
    \label{fig:qa_wo_title}
\end{figure}

==> graphs/70B_RTR.tex <==
\begin{figure}
    \centering
\includegraphics[width=0.45\textwidth]{images/70B_RTR.png}
\vspace{-4mm}
    \caption{\textbf{Effectiveness of RTR for 70B model} }
    \label{fig:70B_RTR}
\end{figure}

==> graphs/answer_position_stats.tex <==
\begin{figure}
    \centering
\includegraphics[width=0.4\textwidth]{images/qa_position_stat.pdf}
    \caption{Histograms of the answer positions. We count how many sentences are before the sentence generating the answer.}
    \label{fig:qa_position}
\end{figure}

==> graphs/compare_supervised.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.45\textwidth]{images/compare_sup.png}
\vspace{-4mm}
    \caption{\textbf{Comparison with supervised models.} A model trained with QA pairs for the new domain (Supervised) outperforms unsupervised models (Plain, RTR), but still suffers from positional bias. Adding RTR on top of the supervised model (Supervised + RTR) significantly improves the recall.}
    \label{fig:compare_sup}
\end{figure}

==> graphs/compare_supervised_zephyr.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.45\textwidth]{images/compare_sup_zephyr.png}
    \caption{\textbf{Experiments on Zephyr.} Obtained results are very similar to those of Llama-2 in the main paper. A model trained with QA pairs for the new domain (Supervised) outperforms unsupervised models (Plain, RTR), but still suffers from positional bias. Adding RTR on top of the supervised model (Supervised + RTR) significantly improves the recall.}
    \label{fig:compare_sup_zephyr}
\end{figure}

==> graphs/graph_modelsize.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.4\textwidth]{images/modelsize.png}
\vspace{-3mm}
    \caption{\textbf{Fine-tuned LLMs suffer from the positional bias in learned documents.} We show the recall (y-axis) and position of the sentence with the answer (x-axis) for models with three parameter sizes. Here, we train them for 4,000 iterations. Fine-tuned LLMs return accurate answers located at the beginning of the documents, but underperform for those at the middle and end.}
    \label{fig:graph_modelsize}
\end{figure}

==> graphs/graph_order.tex <==
\begin{figure}
    \centering
\includegraphics[width=0.35\textwidth]{images/graph_order.png}
\vspace{-4mm}
    \caption{\textbf{Random token replacement (RTR) improves robustness to the position of the answer in the learned documents.} Recall (y-axis) and the position of the sentence with the answer (x-axis). 
    \textit{Plain} model significantly suffers from positional bias. \textit{Shuffle} model shows improvement at the end of the sentence but lowers performance at the beginning. In contrast, \textit{RTR}, \ie, replacing tokens with random ones, shows improvement in all positions.}
    \label{fig:graph_order}
\end{figure}

==> graphs/iterations.tex <==
\begin{figure}
    \centering
\includegraphics[width=0.4\textwidth]{images/iterations.png}
\vspace{-3mm}
    \caption{Longer training increases the effect by the positional bias. We split the questions into three groups by their position in the training document. Longer training improves the performance of the first group while reducing that of the middle and last groups. }
    \label{fig:graph_iterations}
\end{figure}

==> graphs/mask_rate.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=0.35\textwidth]{images/mask_rate.png}
\vspace{-4mm}
    \caption{\textbf{Ratio for random token replacement.} Recall (y-axis) and the position of the answer in the document (x-axis). For simplicity, we categorize 9 questions into 3 groups by their position and show in the x-axis.}
    \label{fig:mask_rate}
\end{figure}

==> graphs/model_size_wiki.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/wiki_perplexity.png} 
  \caption{}
  \label{fig:perplexity}
\end{subfigure}%
\begin{subfigure}{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/wiki_em_model_size_pos.png}
   \caption{}
  \label{fig:em_wiki}
\end{subfigure}
% \begin{subfigure}{0.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{icml2023/images/wiki_f1_position.png}
%   \caption{F1 score on \fontchange{pcr}{Wiki2023+}.}
%   \label{fig:f1_wiki}  
% \end{subfigure}
\caption{\fontchange{pcr}{Wiki2023+}.}
\label{fig:perplexity_modelsize}
\end{figure}


==> graphs/modelsize_crossdomain.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.42\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/wiki_em_model_size_pos.png} 
  \label{fig:em_bios}
\end{subfigure}%
\hspace{20pt}
\begin{subfigure}{0.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/wiki_all_f1_position.png}
  \label{fig:em_wiki}
\end{subfigure}
\caption{Left: Results on 13B and 70B AR models using EM accuracy on \fontchange{pcr}{Wiki2023+}. Right: Cross-domain evaluation in \fontchange{pcr}{Wiki2023+}.}
\label{fig:summary_result}
\end{figure}

==> graphs/perplexity_analysis.tex <==

\begin{wrapfigure}[9]{r}{0.5\textwidth}
\vspace{-20mm}
\begin{center}
\includegraphics[width=0.8\linewidth]{images/wiki_perplexity.png}
\caption{Perplexity computed for each sentence. }
\end{center}
\label{fig:perplexity_per_sentence}
\end{wrapfigure}


% \begin{figure}
% \centering
% \begin{subfigure}{0.5\textwidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{icml2023/images/wiki_perplexity.png} 
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}{0.5\textwidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{icml2023/images/wiki_perplexity.png}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{Perplexity computed for each sentence without previous sentences. }
% \label{fig:perplexity_per_sentence}
% \end{figure}

==> graphs/size_iter.tex <==
\begin{figure}
\centering
 \begin{subfigure}[b]{0.5\linewidth}
  \centering
  \includegraphics[width=\linewidth]{images/modelsize.png}
  \caption{A subfigure}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}[b]{0.5\linewidth}
  \centering
  \includegraphics[width=\linewidth]{images/iterations.png}
  \caption{A subfigure}
  \label{fig:sub2}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:test}
\end{figure}

==> graphs/summary_wiki_bios.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.45\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{images/synth_group_position.png} 
   \caption{EM accuracy on \fontchange{pcr}{bioS}.}
  \label{fig:em_bios}
\end{subfigure}%
\hspace{20pt}
\begin{subfigure}{0.45\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{images/wiki_em_position.png}
   \caption{EM accuracy on \fontchange{pcr}{Wiki2023+}.}
  \label{fig:em_wiki}
\end{subfigure}
% \begin{subfigure}{0.33\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{icml2023/images/wiki_f1_position.png}
%   \caption{F1 score on \fontchange{pcr}{Wiki2023+}.}
%   \label{fig:f1_wiki}  
% \end{subfigure}
\caption{Left: EM accuracy and the position of the answer in documents for \fontchange{pcr}{bioS}. We group nine properties into three groups by their position and plot the average computed within the group. Right: EM accuracy on \fontchange{pcr}{Wiki2023+}.}
\label{fig:summary_result}
\end{figure}

==> graphs/synth_reverse.tex <==
\begin{figure}[h!]
    \centering
\includegraphics[width=0.45\textwidth]{images/synth_reverse_position.png}
    \caption{EM accuracy on reversed \fontchange{pcr}{bioS}. }
    \label{fig:synth_reverse}
\end{figure}

==> tables/answer_sentence_count.tex <==
% \begin{table*}[]
% \scalebox{0.85}{
% \centering
% \begin{tabular}{c||c|c|c|c|c|c|c|c|c|c}
% \toprule
%  \makecell{QA Dataset}   &Birthday & Birthplace & School & Major & Company & Job & Food & Sports & Hobby & Average\\\hline

% &1.02/100&8.59/97.4&5.48/60.0&8.23/90.4&5.93/60.4&6.41/65.2&8.86/97.8&8.82/96.0&5.86/59.2&6.57/80.7\\
% Alpaca&1.00/98.6&1.02/92.4&1.06/48.2&1.01/13.8&1.31/17.6&1.00/21.2&1.00/27.2&1.00/22.4&1.08/11.4&1.05/39.2\\
% Alpaca+Random Word&1.01/99.4&1.05/96.6&1.12/94.4&1.01/80.2&1.78/79.8&1.00/80.2&1.00/89.6&1.00/61.0&1.00/76.6&1.10/84.2\\

% \bottomrule
% \end{tabular}}
% \label{tab:qa_ablate}
% \caption{The effect using QA dataset for fine-tuning. (Number of returned sentences)/(Recall to retrieve correct information) is shown in each cell. Note that all questions can be answered with one sentence, but the model trained without QA dataset returns redundant answers. In summary, the usage of QA dataset enables the model to return concise answers. }
% \end{table*}

\begin{table}[t]
\centering
\scalebox{1.0}{
\begin{tabular}{c|c|c}
\toprule
 \makecell{QA Data}   &Recall $\uparrow$& Count $\downarrow$ \\\hline
None&80.7&6.57\\
Alpaca&39.2&1.05\\
Alpaca+RTR&64.6&1.10\\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{\textbf{The effect of using QA dataset for fine-tuning.} Recall and number of returned sentences are shown.
Note that all questions can be answered with one sentence, but the model trained without the QA dataset returns redundant answers. The usage of the QA dataset enables the model to return concise answers. }
\label{tab:qa_ablate}

\end{table}

==> tables/chat_vs_nochat.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{

\begin{tabular}{c|c|c|c|c}
\toprule
Size &Inst-tuning&Begin & Middle & End \\\hline
\multirow{2}{*}{7B} &&58.4& 12.3&9.5\\\
&\checkmark&\bf{79.7} & \bf{17.5}&\bf{20.3}\\\hline
\multirow{2}{*}{13B} && 64.7& 14.9 & 19.2\\
 &\checkmark&\bf{78.5}& \bf{29.4}&\bf{27.7}\\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{\textbf{Comparison between models with and without instruction-tuning pre-training.} The model pre-trained with instruction tuning outperforms a model trained only with self-supervision by a large margin.}
\label{tab:chat_nochat}
\end{table}

==> tables/length_news_paper.tex <==

\begin{table}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{c|c|c|c|c}
\toprule
 \makecell{Size}  &News & Dataset & Number & Code \\\hline
 7B & 1.03 & 1.04 & 1.01 & 1.97 \\
 13B & 1.01 & 1.00 & 1.01 & 1.65\\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{\textbf{The count of answer sentences returned by trained models for Paper2023 and News2023, measured on models trained with RTR.} Except for Code in Paper2023, the trained models return concise answers.}
\label{tab:length_news_paper}

\end{table}

==> tables/news_summary.tex <==
\begin{table*}[ht]
\centering
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\scalebox{1.0}{
\begin{tabularx}{0.8\textwidth}{c|c|Y|Y|Y|Y|Y|Y}
\toprule
Size &Augmentation&Who &What&Where&When&How&Average     \\\hline
\multirow{3}{*}{7B}&None&44.2&27.4&35.5&37.6&25.0&33.9\\
&Shuffle&34.2\drop{10.0}&28.8\rise{1.4}&30.8\drop{4.7}&33.4\drop{4.2}&21.0\drop{4.0}&29.6\drop{4.3}\\

&RTR&47.0\rise{2.8} & 41.4\rise{14.0}&47.5\rise{12.0}&48.1\rise{10.5}&37.6\rise{12.6} & 44.3\rise{10.4}\\\hline
\multirow{3}{*}{13B} &None&50.2&33.4&45.9&39.7&34.6 &40.8\\
& Shuffle &47.6\drop{2.6}&39.6\rise{6.2}&51.3\rise{5.4}&39.6\drop{0.1}&35.2\rise{0.6}&42.7\rise{1.9}\\
& RTR &53.8\rise{3.6} & 49.4\rise{16.0} & 62.2\rise{16.4} & 55.3\rise{15.6} & 37.6\rise{3.2} & 51.6\rise{10.8} \\
\bottomrule
\end{tabularx}}
\vspace{-3mm}
\caption{\textbf{Results on News2023.} Shuffling significantly harms performance for some questions because re-ordering sentences can destroy the context among sentences. Colored numbers indicate the improvement compared to the \textit{None} model.}
\label{tab:summary_news}
\end{table*}

% \begin{table}[t]
% \scalebox{0.8}{
% \centering
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \toprule
% Size &Augment&Who &What&Where&When&How&Average     \\\hline
% \multirow{3}{*}{7B}&None&\bf{44.2}&27.4&35.5&37.6&25.0&33.9\\
% &Shuffle&34.2&28.8&30.8&33.4&21.0&29.6\\
% &Replace&40.4&\bf{34.4}&\bf{37.5}&\bf{42.6}&\bf{30.8}&\bf{37.1}\\\hline
% \multirow{2}{*}{13B} &None&\bf{50.2}&33.4&45.9&\bf{39.7}&34.6 \\
% & Shuffle &47.6&\bf{39.6}&\bf{51.3}&39.6&\bf{35.2}\\
% \bottomrule
% \end{tabular}}
% \caption{.}
% \label{tab:summary_news}
% \end{table}

==> tables/paper_summary.tex <==
\begin{table}[t]
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\scalebox{0.9}{
\centering
\begin{tabularx}{0.5\textwidth}{c|c|Y|Y|Y}
\toprule
Size &Augmentation&Dataset &Number&Code\\\hline
\multirow{3}{*}{7B}&None&8.8&7.8&10.6\\
&Shuffle&21.3\rise{12.5}&10.4\rise{2.6}&10.6\rise{0.0}\\
&RTR&19.0\rise{10.2} & 16.8\rise{9.0}& 24.0\rise{13.4}\\\hline
%&Replace&13.2\rise{4.4}&11.1\rise{3.3}&22.0\rise{11.4}\\\hline
\multirow{3}{*}{13B} &None& 22.6&13.9&26.8 \\
&Shuffle&38.0\rise{15.4}&15.8\rise{1.8}&27.8\rise{1.0}\\
&RTR&28.5\rise{5.9}&21.8\rise{7.9}&27.4\rise{0.6}\\
\bottomrule
\end{tabularx}}
\vspace{-3mm}
\caption{\textbf{Results on Paper2023.} Applying data augmentation improves the performance on three types of questions. Colored numbers indicate the improvement compared to the \textit{None} model.}
\label{tab:summar_paper}
\end{table}

==> tables/property_variation.tex <==
\begin{table}[h!]
    \centering
    \small
    \begin{tabular}{c|c}
        \toprule
         QA    & No. of variations \\
        \midrule
      Birthplace & 1115 \\
      School & 2010\\
      Major & 1750\\
      Company & 2434\\
      Occupation & 646\\
      Sports & 224\\
      Food & 294\\
      Hobby & 315\\

        \bottomrule
    \end{tabular}
    \caption{The number of variations in nine properties of our synthetic dataset.}  
    \label{tab:nine_prop_stats}
\end{table}

==> tables/qa_dataset.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{c|c|c|c|c}
\toprule
QA dataset & QA pairs &Begin & Middle & End \\\hline
Flan &0.8M&47.5&13.3&16.8\\
Flan small &0.08M&49.8&16.9&10.6\\
Alpaca &0.05M&\textbf{79.7}&\textbf{17.5}&\textbf{20.3}\\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{\textbf{The choice of the external QA dataset varies the performance a lot.} We show the recall for three groups of questions.}
\label{tab:qa_dataset}
\end{table}

==> tables/qa_ex.tex <==

\begin{table*}[t]
    \centering
    \small
    \scalebox{0.85}{
    \begin{tabular}{c|c|c|c}
        \toprule
Dataset    & Q-Type &Question & Answer \\
       \midrule
     %Alcuna & Habitat, Harvest, Leaf Mass per Area\\
\multirow{2}{*}{SynthBio} &Birthday& When was Karim Ali Jr. born ?     &  November 11, 2020.\\
& Workplace& Where Karim Ali Jr. was employed? & Belmopan, Belize \\\hline    
  \multirow{2}{*}{News} & Who & Who is currently considered the most indispensable player on the Packers roster? & Christian Watson\\      
   & When & When is the game between the Titans and Steelers scheduled? & November 2, 2023, at 8:15 PM ET.\\\hline
     
   \multirow{2}{*}{Paper} & Dataset & Which dataset is used for evaluation? & COCO Dataset\\
    & Number & How many node classification benchmarks does AERO-GNN outperform baseline GNNs on? & 9 out of 12\\
        \bottomrule
    \end{tabular}}
    \caption{QA examples.}
    \label{tab:question_examples}
\end{table*}

==> tables/qa_news_stats.tex <==
\begin{table}
    \centering    
    \begin{tabular}{c|c}
        \toprule
         QA    & No. of questions \\
        \midrule
      Who & 500\\
      What & 500 \\
      Where & 259\\
      When & 401\\
      How & 500\\
        \bottomrule
    \end{tabular}
    \caption{Stats of QA pairs for News2023 datasets.}  
    \label{tab:qa_news_stats}
\end{table}


==> tables/qa_paper_stats.tex <==
\begin{table}
    \centering
    \small
    \begin{tabular}{c|c}
        \toprule
         QA    & No. of questions \\
        \midrule
      Dataset & 715\\
      Code & 500\\
      Number & 653 \\
      Question w/o paper title & 479\\
        \bottomrule
    \end{tabular}
    \caption{Stats of QA pairs for Paper2023 datasets. }  
    \label{tab:qa_paper_stats}
\end{table}

==> tables/qa_stats.tex <==
\begin{table}[!h]
\begin{minipage}{.5\linewidth}
\centering
    \begin{tabular}{c|c}
        \toprule
         QA    & No. of questions \\
        \midrule
      Dataset & 715\\
      Code & 500\\
      Number & 653 \\
      Question w/o paper title & 479\\
        \bottomrule
    \end{tabular}   
    \end{minipage}%
\begin{minipage}{.5\linewidth}
\centering
    \begin{tabular}{c|c}
        \toprule
         QA    & No. of questions \\
        \midrule
      Who & 500\\
      What & 500 \\
      Where & 259\\
      When & 401\\
      How & 500\\
        \bottomrule
    \end{tabular}
     \end{minipage}%
      \caption{Stats of QA pairs for Paper2023 datasets (Left) and News2023 datasets (Right).}  
    \label{tab:qa_stats}
   \end{table}


==> tables/qa_summary.tex <==

\begin{table}[t]
    \centering
    \small
    \scalebox{1.0}{
    \begin{tabular}{c|cc}
        \toprule
     Dataset &Question Types&  \\
       \midrule
      \multirow{3}{*}{SyntheticBio}  & Birthday, Birthplace, School \\
      & Major, Company, Occupation \\ 
      & Food, Sports, Hobby \\\hline
     News2023 & Who, Where, When, What, How\\ \hline
     Paper2023 & Dataset, Number, Code location   \\       
        \bottomrule
    \end{tabular}}
    \caption{Types of questions.}
    \label{tab:qa_dataset}
\end{table}


==> tables/stats_dataset.tex <==
\begin{table}[h!]
    \centering
    \small
    \begin{tabular}{c|c|c}
        \toprule
         Dataset    & Docs      & Tokens per Doc \\
        \midrule
       SynthBio &3000&169.5\\
        News2023 & 1,937 & 406.8\\
        Paper2023 & 7,232 & 265.8\\
        \bottomrule
    \end{tabular}
    \caption{Stats of documents datasets. }  
    \label{tab:dataset_stats}
\end{table}



==> tables/stats_evaluation.tex <==
\begin{table}[h!]
\centering
\scalebox{0.85}{
\begin{tabular}{|l|c|c|c|}\hline
\backslashbox{Human}{ChatGPT}
&Correct & Partially correct & Incorrect\\\hline
Correct &193&55&0\\\hline
Partially correct &6 & 135 & 4\\\hline
Incorrect &4& 188 & 128\\\hline
\end{tabular}}
 \caption{We manually annotate the correctness of LLM's generated answer for Paper2023 and compare its alignment with ChatGPT.}  
    \label{tab:eval_stats}
\end{table}

==> tables/synth_summary.tex <==
\begin{table*}[h]
\scalebox{0.9}{
\centering
\begin{tabular}{c|c|c||c|c|c|c|c|c|c|c|c||c}
\toprule
Size &Shuffle& \makecell{ Prompt \\ Aug }&Birthday & Birthplace & School & Major & Company & Job & Food & Sports & Hobby & Mean     \\\hline
&&&98.6     & 92.4       & 48.2   & 13.8  & 17.6    & 21.2       & 27.2 & 22.4   & 11.4  & 39.2        \\
7B&\checkmark&&26.0       & 41.0         & 41.2   & 32.0    & 31.0      & 34.2       & 25.2 & 32.6   & 23.0    & 31.8        \\
&&\checkmark&99.4     & 85.4       & 47.8   & 24.6  & 21.4    & 17.6       & 29.6 & 24.6   & 13.8  & 40.5\\\hline

 &&&100&82.6&52.8&10.2&52.0&26.0&35.2&27.4&20.6&45.2\\
13B &\checkmark&& 39.4 & 49.4 & 46.4 & 32.0 &42.0&31.4&38.4&39.4&35.4&39.3\\

 & & \checkmark& 93.2&77.4&50.6&25.6&46.2&30.6&	37.8&33.8&27.6&46.9\\
\bottomrule
\end{tabular}}
\caption{Summary of experiments on the synthetic biography dataset. Surprisingly, the trained model can answer some types of questions, e.g., Birthday and Birthplace, very accurately. The result indicates that I-LLM can retrieve information embedded in the unlabeled document even without being trained with question-answer pairs about the information.}
\label{tab:summary_synth}
\end{table*}

==> tables/title.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{c|c|c|c}
\toprule
Trained with tag& Birthday & Job & Average \\\hline
 &95.0&8.6&38.0\\\
\checkmark&\textbf{98.6}&\textbf{21.2}&\textbf{39.2}\\
\bottomrule
\end{tabular}
\caption{Comparison between models with and without tag of items. We train a model on synthetic documents which exclude the tag of items, e.g., Birthday, School of education, as shown in Fig.~2 in the main paper. Tagging a sentence should clarify what is described in each sentence. For a question about a job, tagging significantly improves performance. }
\label{tab:tag_notag}
\end{table}

==> tables/zephyr_compare.tex <==
\begin{table*}[t]
\centering
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\scalebox{1.0}{
\begin{tabularx}{0.8\textwidth}{c|c|Y|Y|Y|Y|Y|Y}
\toprule
Model &Augmentation&Who &What&Where&When&How&Average     \\\hline
\multirow{2}{*}{Llama-2} &None&44.2&27.4&35.5&37.6&25.0&33.9\\
&RTR&47.0\rise{2.8} & 41.4\rise{14.0}&47.5\rise{12.0}&48.1\rise{10.5}&37.6\rise{12.6} & 44.3\rise{10.4}\\\hline
\multirow{2}{*}{Zephyr} &None&40.2&32.6&37.6&37.4&27.8&35.1\\
&RTR&35.6\drop{-4.6}& 37.6\rise{5.0}& 32.0\drop{-5.6}& 35.9\drop{-1.5}& 32.4\rise{4.6}& 34.7\drop{-0.4}\\
\bottomrule
\end{tabularx}}
\vspace{-3mm}
\caption{\textbf{Comparison between LLama-2 and Zephyr in News2023.}}
\label{tab:zephyr_news}
\end{table*}


